Intrinsic Rowhammer PUFs: Leveraging the Rowhammer Effect for Improved Security

Physically Unclonable Functions (PUFs) have become an important and promising hardware primitive for device fingerprinting, device identification, or key storage. Intrinsic PUFs leverage components already found in existing devices, unlike extrinsic silicon PUFs, which are based on customized circuits that involve modification of hardware. In this work, we present a new type of a memory-based intrinsic PUF, which leverages the Rowhammer effect in DRAM modules; the Rowhammer PUF. Our PUF makes use of bit flips, which occur in DRAM cells due to rapid and repeated access of DRAM rows. Prior research has mainly focused on Rowhammer attacks, where the Rowhammer effect is used to illegitimately alter data stored in memory, e.g., to change page table entries or enable privilege escalation attacks. Meanwhile, this is the first work to use the Rowhammer effect in a positive context: to design a novel PUF. We extensively evaluate the Rowhammer PUF using commercial, off-the-shelf devices, not relying on custom hardware or an FPGA-based setup. The evaluation shows that the Rowhammer PUF holds required properties needed for the envisioned security applications, and could be deployed today.

==> relatedwork.tex <==
\section{Related Work}
\label{sec:related}

The Rowhammer effect was first exposed by Kim et al.~\cite{kim2014flipping} by repeatedly and rapidly toggling DRAM wordlines in order to induce bit flips in adjacent DRAM locations. Using an FPGA testbed the authors conducted extensive experiments and showed the prevalent existence of disturbance error in various commodity DRAM chips. A recent report demonstrated the existence of DRAM disturbance errors in recent DDR4~\cite{DDR4} modules as well.
%Previous literature required the existence of cache flush instructions (i.e., $\mathtt{CLFLUSH}$) in order to circumvent CPU caching mechanisms, ensuring direct access to DRAM. Gruss, et al.~\cite{gruss2015rowhammer} and Aweke, et al.~\cite{aweke2016anvil} introduced the first means to induce DRAM disturbance error without relying on the cache flush instruction by forcing cache eviction through elaborate memory access patterns. Qiao et al.~\cite{Qiao2016} showed that x86 non-temporal store instructions, which do not use the CPU cache, can be exploited to trigger Rowhammer. In~\cite{veen:2016}, Veen, et al. exploited non-cacheable DMA accesses to show Rowhammer effects.
In case of the platforms without the cache line flush instruction (i.e., $\mathtt{CLFLUSH}$), in order to circumvent CPU caching mechanisms and ensure direct access to DRAM, Gruss, et al.~\cite{gruss2015rowhammer} and Aweke, et al.~\cite{aweke2016anvil} force cache eviction through elaborate memory access patterns, Qiao et al.~\cite{Qiao2016} make use of x86 non-temporal store instructions, which do not use the CPU cache, and Veen, et al.~\cite{veen:2016} exploited non-cacheable DMA accesses to show Rowhammer effects.
Razavi et al.~\cite{razavi2016flip} presented a technique that allows for targeted bit flips over arbitrary physical memory locations. In order to conduct predictable Rowhammer attacks, \cite{veen:2016} uses a brute-force approach to hammer all DRAM rows and collect information about predictable bit flip locations. In the work of Jung et al.~\cite{jung2016reverse} a novel approach is presented that allows for reconstructing the physical layout of DRAM cells, by applying multiple temperature gradients on the memory module and observing DRAM data retention, which can further aid with Rowhammer.

The Rowhammer effect has been used for implementing various practical security exploits. In~\cite{seaborn2015exploiting} and~\cite{veen:2016}, the authors rely on Rowhammer effect to gain root privileges by flipping bits in page table entries (PTEs). 
%Xiao et al.~\cite{xiao2016one} use Rowhammer in cross-virtual machine settings in order to attack Xen's paravirtualized memory isolation by employing Rowhammering from within a malicious virtual machine. 
Xiao et al.~\cite{xiao2016one} attack Xen's paravirtualized memory isolation by employing Rowhammering from within a malicious virtual machine. 
In~\cite{razavi2016flip} and~\cite{bhattacharya2016curious}, authors successfully attack RSA by creating bit flips in keys stored in DRAM. The authors of~\cite{aichinger2015ddr} and~\cite{aweke2016anvil} showed that ECC and doubled DDR refresh rates are not enough to mitigate the Rowhammer attack.

%Researchers have discovered several ways to do Rowhammer without the CLFLUSH instruction. Gruss et al.~\cite{gruss2015rowhammer} and Aweke et al.\cite{aweke2016anvil} demonstrated that using a cache eviction strategy to flush the aggressor row and trigger the Rowhammer bug. 
%The Rowhammer bug has been exploited for several attacks. In \cite{seaborn2015exploiting, veen:2016}, user programs can escape sandbox by flipping bits to change control flow and get root privilege by flipping bits in page table entries. In \cite{xiao2016one}, malicious VM use Rowhammer to crack memory isolation in Xen. 
%To conduct predictable Rowhammer attack, \cite{veen:2016} uses brute force to hammer all DRAM rows and collect information about useful bit flips.
%In \cite{razavi2016flip, bhattacharya2016curious}, authors successfully attack RSA by creating bit flips in keys stored in DRAM.
%An empirical approach in \cite{veen:2016} uses brute force to hammer all DRAM rows and collect information about which bits will flip when certain row is hammered.  
%This knowledge of the physical address location of the bit flip is sufficient to allow designing an attack that flips bits in page table entries of the OS, to eventually gain root privileges by being able to write to kernel memory due to corrupted page tables.
%Researchers have looked at extraction of the exact location of each DRAM cell in a DRAM array in order to enhance the Rowhammer attack \cite{jung2016reverse}.  They have reversed-engineered the DRAM by adding a thermal gradient to DRAM chip to get insights into the physical bit location.


%?Time Measurements and Modelling of Bit Error Rates of WIDE I/O DRAM in MPSoCs?

